Temporal Sequencing of Documents

We outline an unsupervised method for temporal rank ordering of sets of historical documents, namely American State of the Union Addresses and DEEDS, a corpus of medieval English property transfer documents. Our method relies upon effectively capturing the gradual change in word usage via a bandwidth estimate for the non-parametric Generalized Linear Models (Fan, Heckman, and Wand, 1995). The number of possible rank orders needed to search through for cost functions related to the bandwidth can be quite large, even for a small set of documents. We tackle this problem of combinatorial optimization using the Simulated Annealing algorithm, which allows us to obtain the optimal document temporal orders. Our rank ordering method significantly improved the temporal sequencing of both corpora compared to a randomly sequenced baseline. This unsupervised approach should enable the temporal ordering of undated document sets.

==> code.tex <==
{\tiny
\begin{verbatim}

IN THIS PROGRAM, WE SELECTED 100 RANDOM SAMPLES, WHERE EACH SAMPLE CONSISTS OF A SEQUENCE OF
TEN ADDRESSES FROM STATE OF THE UNION ADRESS (SOTU) THAT ARE DATED TO BE 23 YEARS APART 
(RANGING FROM 1790 TO 2020). WE RANDOMLY PERMUTE THE TEMPORAL ORDER OF THE SEQUENCE OF THE TEN
ADDRESSES FROM EACH SAMPLE, WHICH ARE THE INPUTS, AND 
THE OUTPUTS ARE THE TRUE TEMPORAL ORDER PREDICTIONS OF EACH ONE OF THE PERMUTED SAMPLES. 
############################################################################################### 
###############################################################################################


                    ############## PRE-PROCESSING OF TEXTUAL DATA ##############
//Input: From the SOTU corpus, read all lines (each line being an Address) into an array
SofUtext = read lines from file=SOTU into an array

// Determine the length of the input text array which is equal the total number of Addresses
L = length(SofUtext)

// Create a copy of the input text array
SofU2gramtxt = SofUtext

// Iterate over each element in the array
for i from 1 to L do
    // Extract the current text element
    s = SofU2gramtxt[i]
    
    // Split the current text element into words
    w = split s into words using space as delimiter
    
    // Generate n-grams (here, unigrams) from the words
    ngrams_list = generate n-grams from w with n = 1
    
    // Join the n-grams with underscores and update the text element in the array
    updated_text = join ngrams_list with underscores
    SofU2gramtxt[i] = updated_text
end for

// Convert the text data into a Document-Term Matrix
DocTermMatrix = create Document-Term Matrix from SofU2gramtxt

// Convert the Document-Term Matrix to a matrix format
SofUVCDocTerm = convert DocTermMatrix to matrix format

// Remove corrupted or non-words from the columns. (We removed the first 1254 columns) 
SofUVCDocTerm = remove columns 1 to 1254 from SofUVCDocTerm

// Find columns (terms) where the sum of entries is greater than or equal to 2
indx = find column indices where sum of entries >= 2

// Filter the matrix to keep only the relevant columns
SofUVCDocTerm = keep columns with indices in indx from SofUVCDocTerm

// Transpose the matrix (swap rows and columns) and assign the transposed matrix to FreqTableSofU
FreqTableSofU = transpose SofUVCDocTerm

                            
##################### SAMPLE 100 TIMES A SEQUENCE OF 10 ADDRESSES 23 YEARS APART. ENSURE THAT THERE ARE NO DUPLICATED SAMPLES BY 
SAMPLING 200 TIMES, THEN REMOVING THE DUPLICATED TERMS, AND THEN SAVING THE FIRST 100 UNDUPLICATED SAMPLES. THE UNIQUE 
100 SAMPLES ARE STORED IN MATRIX "SampleMat" #####################

// Set column names of the matrix "FreqTableSofU" to be sequential numbers starting from 1
through number of columns

// Define constants
lengthofstring = 10
numofspeech = number of columns in FreqTableSofU

// Set the number of samples to extract
numSample = 200

// Initialize a matrix to store sample data with zeros
SampleMat = create matrix with numSample rows and lengthofstring columns, filled with zeros

// Initialize count variable
count = 1

// Continue sampling until the count exceeds numSample
while count <= numSample do
    // Select an initial sample index randomly from the range 1 to numofspeech
    initialsample = random integer between 1 and numofspeech

    // Generate a sequence of indices for the sample
    SampleSofU = create sequence starting at initialsample and incrementing by 23, with length equal to lengthofstring
    SampleSofU = take modulo numofspeech for each element in the sequence

    // Handle indices where the result is 0
    indx = find indices in SampleSofU where value is 0
    if length of indx > 0 then
        // Set these indices to 240
        set elements in SampleSofU at indx to 240

    // Sort the sample indices
    SampleSofU = sort SampleSofU

    // Store the sorted sample into the matrix SampleMat
    SampleMat[count, ] = SampleSofU
    
    // Increment the count
    count = count + 1
end while

// Set the number of unique samples to keep
numSampleNow = 100

// Ensure SampleMat contains only unique rows and keep only the first numSampleNow rows
SampleMat = get unique rows from SampleMat
SampleMat = keep the first numSampleNow rows of the unique rows of SampleMat


                                        ####### MAIN FUNCTION #######
######################  WITHIN EACH FOR LOOP:  EACH ROW OF THE SAMPLE MATRIX "SampleMat" CONSISTS OF A SET OF 10 RANDOM ADDRESSES 23 YEARS APART. 
IN THE MATRIX "FreqMatrixFinal", THE COLUMNS CORRESPOND TO A TEMPORALLY ORDERED SAMPLED ADDRESSES, AND THE ROWS ARE WORDS WHICH 
HAVE OCCURRED ACROSS THE SAMPLED ADDRESSES AT LEAST TWICE. AN ELEMENT OF THE MATRIX IS THE COUNT OF A WORD (ROW) IN THE COLUMN ADDRESS. 
"Sint" IS A RANDOM PERMUTATION OF THE COLUMNS OF "FreqMatrixFinal". THE INPUT FOR THE SIMULATED ANNEALING ALGORITHM IS THE MATRIX 
"FreqMatrixFinal" ALONG WITH THE RANDOM COLUMN PERMUTATION "Sint". THE OUTPUT IN THE ROW OF THE MATRIX "SestHopt" IS THE PREDICTED 
ORDER PRIOR TO THE PERMUTATION BY "Sint". ######################

// Create a matrix to store results with numSampleNow rows and lengthofstring + 1 columns
SestHopt = create matrix with numSampleNow rows and (lengthofstring + 1) columns, filled with zeros

// Loop through each sample
for i from 1 to numSampleNow do
    // Extract the i^th row from SampleMat
    S = SampleMat[i, ]

    // Extract relevant columns from FreqTableSofU based on indices S
    FreqMatrixTemp = extract columns from FreqTableSofU using S

    // Find rows in FreqMatrixTemp where the sum of values is at least 2
    IndxRow = find row indices where sum of values >= 2

    // Filter the matrix to keep only the relevant rows
    FreqMatrixFinal = keep rows in FreqMatrixTemp at IndxRow

    // Get the number of elements in S
    M = length of S

    // Randomly permute the sequential order of S
    Sint = A string of random permutation of the integers between 1 and M


    // Apply SimAnnealHopt function to the filtered frequency matrix and the sampled index
    SestHopt[i, ] = result of SimAnnealHopt(FreqMatrixFinal, Sint)

    // Prepare the output vector including the index and results
    x = concatenate i with SestHopt[i, ]

    // Write the output to a file with specified format. 
    // The first column is the index. The second column is the bandwith associated with the predicted temporal order 
    //(Section 5.1, equation (4)). 
    // The remaining 10 columns are the estimated order of the true temporal (the correct order is 1 to M sequentially, M=10)
    
    write x to file ="SestHopt.txt", with 12 columns, in append mode
end for




############# SUB-FUNCTION: COMPUTES THE ELEMENTS REQUIRED TO COMPUTE BANDWIDTH (EQUATION 11 AND EQUATION B IN APPENDIX B) ###########
Function HoptInputFun():
    // Define degrees of freedom for the t-distribution
    nu <- 5
    
    // Generate 10000 random variables from a t-distribution with 'nu' degrees of freedom
    xrand <- GenerateRandomTDistribution(10000, nu)
    
    // Compute the density of the t-distribution at the generated random variables
    densities <- ComputeDensity(xrand, nu)
    
    // Calculate the mean of the densities (this is the last component of equation 11 in Appendix B (\int K^2(z)dz)).
    IntgKsqrd <- Mean(densities)
    
    // Calculate the second moment squared for the t-distribution 
    //(this is the first component of equation B in Appendix B ( (\int z^2K(z)dz)^2 ) )
    secMomentSqr <- (nu / (nu - 2))^2
    
    // Return the results as a list or array
    Return [IntgKsqrd, secMomentSqr]
    

        ############# SUB-FUNCTION: COMPUTING THE MEDIAN AVERAGE BANDWIDTH VALUE ACROSS WORDS (SECTION 5.1, EQUATION 3) #############
function HoptFun(FreqMatrixFinal, Sint) 
    // Get the necessary input values for the function
    hoptInput = call HoptInputFun()
    IntgKsqrd = hoptInput[1]
    secMomentSqr = hoptInput[2]

    // Initialize variables
    d1 = number of rows in FreqMatrixFinal
    hoptArray = create an array of length d1 filled with zeros
    x = create a sequence from 1 to length of Sint
    N = compute column sums of FreqMatrixFinal for columns specified by Sint
    M= length of Sint   
    
    // Loop through each row of FreqMatrixFinal
    for i from 1 to d1 do
        // Compute x squared
        x2 = x squared

        // Create matrix of trials with observed counts of success and faliure 
        Trials = combine FreqMatrixFinal[i, Sint] with (N - FreqMatrixFinal[i, Sint])

        // Fit a logistic regression model to the trials data
        model = fit a generalized linear model with Trials ~ x + x2 using binomial(link="logit")

        // Calculate the second derivative of the log-likelihood function
        nu2ndderivArray = 2 * model$coefficients[3]

        // Compute the squared second derivative
        Expnu2ndderivArray = nu2ndderivArray squared

        // Calculate the inverse variance
        invVar = sum of (model$fitted values * (1 - model$fitted values))^-1

        // Compute hopt using the formula
        hopt = (IntgKsqrd * invVar / (secMomentSqr * Expnu2ndderivArray * M))^(1/5) 

        // Store the result in the array
        hoptArray[i] = hopt
    end for

    // Return the median of the hoptArray 
    return median of hoptArray
end function


########## SUB-FUNCTION: CREATE A NEIGHBOURHOOD FROM THE CURRENT INPUT SEQUENCE BY REVERSING AND/OR 
MOVING A SUBSEQUENCE OF TERMS (SECTION 5.2) #############
function CreateneighbourSolNew(S) 
    // Get the length of the input sequence
    M = length of S

    // Randomly select an anchor index and define the subsequence to be moved
    anchorIndx = random integer between 1 and (M - 3)
    indextake = sequence from anchorIndx to (anchorIndx + 3)

    // Randomly select an index where the subsequence will be placed
    dropIndx = random integer between 1 and (M - 3)
    indexput = sequence from dropIndx to (dropIndx + 3)

    // Create a new sequence to be modified
    SNew = create a numeric array of length M initialized to zeros

    // Place the subsequence into the new position
    SNew[indexput] = S[indextake]

    // Copy the remaining elements
    SNew[-indexput] = S[-indextake]

    // Randomly decide whether to reverse the order of the moved subsequence
    flip = random integer from the set {0, 1}
    if flip equals 1 then
        // Reverse the order of the subsequence in the new sequence
        LenI = length of indexput
        SNew[indexput] = SNew[indexput reversed]

    // Return the modified sequence
    return SNew
end function


                    ########## SUB-FUNCTION: ANNEALING SCHEDULE ########## 
function CalculateTemp(Constant, i)
    // Calculate the temperature based on the given constant and index
    Temp = Constant raised to the power of (-i)
    
    // Return the calculated temperature
    return Temp
end function


                    ########## SUB-FUNCTION: A CALL FROM THE SUB-FUNCTION "SIMULATED ANNEALING" ##########
function EntropySeqHopt(FreqMatrixFinal, S)
    // Call HoptFun with FreqMatrixFinal and S and negate the result. 
    hopt = - call HoptFun(FreqMatrixFinal, S)
    
    // Return the computed entropy value
    return hopt
end function

############### SUB-FUNCTION: SIMULATED ANNEALING ALGORITHM. WHEN SEEN IN CONJUCTION WITH THE SUB-FUNCTION "EntropySeqHopt", THIS ALGORITHM FINDS 
A SEQUENCE SOLUTION THAT MAXIMIZES THE MEDIAN AVERAGE BANDWIDTH VALUE ACROSS WORDS (SECTION 5.1, EQUATION 4). ######################

function SimAnnealHopt(FreqMatrixFinal, Sint)
    // Initialize parameters
    Constant = 1.011
    Scurrent = Sint
    Sbest = Scurrent
    i = 1

    // Iterate to perform simulated annealing
    while i <= 150 do
        i = i + 0.5

        // Generate a new neighboring solution
        Si = call CreateneighbourSolNew(Scurrent)

        // Calculate current temperature
        tempcurrent = call CalculateTemp(Constant, i)

        // Compute entropy for current and new solutions
        EntropySeqSi = call EntropySeqHopt(FreqMatrixFinal, Si)
        EntropySeqScurrent = call EntropySeqHopt(FreqMatrixFinal, Scurrent)
        
        // Calculate the change in entropy
        deltaEntropy = EntropySeqSi - EntropySeqScurrent

        // Evaluate if the new solution is better
        if deltaEntropy < 0 then
            Scurrent = Si
            // Update the best solution if the new one is better
            if EntropySeqSi <= call EntropySeqHopt(FreqMatrixFinal, Sbest) then
                Sbest = Si
            end if
        else
            // Accept the new solution with a certain probability
            if exp(-deltaEntropy / tempcurrent) > random value between 0 and 1 then
                Scurrent = Si
                // Print details if the new solution is accepted
                print exp(-deltaEntropy / tempcurrent) 
                print tempcurrent
            end if
        end if
    end while

    // Compute the optimal bandwith value for the best ordering solution
    h = - call EntropySeqHopt(FreqMatrixFinal, Sbest)

    // Return the result as a vector
    return vector containing h and Sbest
end function

\end{verbatim}


\begin{comment}

library(topicmodels)
library(tidytext)
library(dplyr)
library(tm)
library(ggplot2)
library(tidyverse)
library(tidygraph)
library(np)

############################################
# THIS PROGRAM TAKES 10 DOCUMENTS THAT ARE 15 YEARS APPART, FROM 1790 TO 2019, AND EXTRACTS
# THE WORDS THAT ARE REPEATED AT LEAST TWICE. THE MATRIX FreqMatrix CONTAINS THE REPEATED WORDS ALONG THE
# ROWS AND THE COLUMNS CORRESPOND TO THE 10 DOCUMENTS.
#########################################################################################
##########################################################################################               (1a)
'''
SofUtext<-readLines("/home/tilahung/Ordering/SofU", n=-1)
L<-length(SofUtext); SofU2gramtxt<-SofUtext

for(i in 1:L){
    s<-SofU2gramtxt[i]
    w<-strsplit(s, " ", fixed = TRUE)[[1L]]  ## Split into words:
    SofU2gramtxt[i]<-paste(vapply(ngrams(w, 1L), paste, "", collapse = "_"), sep=" ", collapse = " ")
}

SofUVCDocTerm<-as.matrix(DocumentTermMatrix(VCorpus(VectorSource(SofU2gramtxt))))
SofUVCDocTerm<-SofUVCDocTerm[, -(1:1254)]  # the terms from 1:1252 are "useless" types

indx<-which(colSums(SofUVCDocTerm)>=2)
SofUVCDocTerm<-SofUVCDocTerm[,indx]

SofUVCDocTerm<-t(SofUVCDocTerm)

FreqTableSofU<-SofUVCDocTerm
VocSofU<-colnames(FreqTableSofU); LVocSofU<-length(VocSofU)

'''
FreqTableSofU<-as.matrix(read.csv("/home/tilahung/Ordering/frequency-matrix.csv")) #cols speech, rows vocabulary
colnames(FreqTableSofU)={}
vocSofU<-read.csv("/home/tilahung/Ordering/vocabulary.csv") #voc correspnding to rows of freqTableSofU 
yearsofinterest<-seq(1790,2019,1) #date range of speeches
'''

FreqTableSofU<-as.matrix(read.table("/home/tilahung/Ordering/FreqTableSofU"))
colnames(FreqTableSofU)={}
VocSofU<-read.table("/home/tilahung/Ordering/VocSofU")
rownames(FreqTableSofU)<-VocSofU$V1

'''

        ######################  Main Program ##################





#  GIVEN A SEQUENCE S, COMPUTE THE PROBABILITY OF OCCURRENCE OF THE DOCUMENTS AT EACH "TIME" POINT
# THIS PORTION OF THE PROGRAM NEEDS TO BE WRITTEN AS A FUNCTION THAT GETS USED BY THE SIMULATED
# ANNEALING ALGORITHM


FreqTableSofU<-as.matrix(read.table("/home/tilahung/Ordering/FreqTableSofU", header=TRUE))
colnames(FreqTableSofU)=1:dim(FreqTableSofU)[2]

lengthofstring<-10;  numofspeech<-dim(FreqTableSofU)[2]  #18217 X 240
numSample<- 200; SampleMat<- matrix(0,numSample,lengthofstring)
count=1

while(count<=numSample){
         initialsample<-sample(1:numofspeech,1)
         SampleSofU<-c(initialsample, initialsample+(1:(lengthofstring-1))*23)%%(numofspeech)
         indx<-which(SampleSofU==0)
         if(length(indx)>0){
             SampleSofU[indx]=240
         }
         SampleSofU<-sort(SampleSofU) 
         SampleMat[count,]<-SampleSofU
         count=count+1
}


numSampleNow<-100
SampleMat<-unique(SampleMat)[1:numSampleNow,]
SestHopt<-matrix(0,numSampleNow,lengthofstring+1) #columns is now 11; hoptimal &length of 10 strings 


for(i in 1:numSampleNow){  #starts from 1
    S<-SampleMat[i,]
    FreqMatrixTemp<-FreqTableSofU[,S]
    IndxRow<- which(rowSums(FreqMatrixTemp)>=2)
    FreqMatrixFinal<- FreqMatrixTemp[IndxRow,]			
    M<-length(S)
    Sint=sample(1:M); print(c("Sint=", Sint))
    SestHopt[i,]<-SimAnnealHopt( FreqMatrixFinal, Sint)
    print(SestHopt[i,])
    x=c(i, SestHopt[i,])
    write(x,file="/home/tilahung/Ordering/SestHoptNewV3.txt",ncolumns =12, append=TRUE, sep = " ")
}

write.table(SampleMat,"SampleMatSofU",row.names = FALSE, col.names = FALSE)
########################  Bandwidth HoptFun Input ##############################

HoptInputFun<-function(){
    nu<-5
    xrand<-rt(10000,nu)   #1000 random variables from a t-distribution 
    IntgKsqrd<-mean(dt(xrand, nu))
    secMomentSqr<- (nu/(nu-2))^2
    return(c(IntgKsqrd,secMomentSqr))
}
    


########################  Bandwidth  Function ##############################
HoptFun<-function( FreqMatrixFinal, Sint){

    hoptInput<-HoptInputFun()
    d1<- dim(FreqMatrixFinal)[1]
    IntgKsqrd<-hoptInput[1]
    secMomentSqr<-hoptInput[2]
    
    hoptArray<-numeric(d1)
    x<-1:length(Sint)
    N<-colSums(FreqMatrixFinal[,Sint])
    
    for(i in 1:d1){
        x2<-x^2
        Trials<-cbind(FreqMatrixFinal[i,Sint],N-FreqMatrixFinal[i,Sint] )
        model<-glm(Trials~x+x2, family = binomial(link="logit")) 
        nu2ndderivArray<- 2*model$coefficients[3]
        Expnu2ndderivArray<-nu2ndderivArray^2
        #invVar<-sum( ( (1/N)*model$fitted*(1-model$fitted) )^{-1} )
        #hopt<-{ (IntgKsqrd*invVar)/(10*secMomentSqr*Expnu2ndderivArray)}^{1/5}
	invVar<-sum( ( model$fitted*(1-model$fitted) )^{-1} )
        hopt<-{ (IntgKsqrd*invVar)/(secMomentSqr*Expnu2ndderivArray)}^{1/5}
        hoptArray[i]<-hopt
    }
    #print(hopt)
    return(median(hoptArray))
}

		

################ FINDING NEIGHBOURHOOD OF A SEQUENCE  ##################                (6)

CreateneighbourSolNew<-function(S){ # this is the PS6 from Tiang paper. The length of the sunsequence is set at 4
    M<-length(S)
    anchorIndx<-sample(1:(M-3),1)
    indextake<-anchorIndx:(anchorIndx+3)

    dropIndx<-sample(1:(M-3),1)
    indexput<-dropIndx:(dropIndx+3)

    SNew<-numeric(M)
    SNew[indexput]<-S[indextake]
    SNew[-indexput]<-S[-indextake]

    flip<-sample(c(0,1),1); # to reverse order
    if(flip==1){
        LenI<-length(indexput)
        SNew[indexput]<-SNew[indexput[LenI:1]]
    }
    return(SNew)
}    



##################################### ANNEALING SCHEDULE ###############################       (7)

CalculateTemp<-function(Constant,i){
	return(Constant^{-i})
}



################### THIS COMPUTES THE AGGREGATE ENTROPY OF A SEQUENCE  #######################   (8)



EntropySeqHopt<-function(FreqMatrixFinal,S){  #formerly WordVarFun function (see "OrderingMergeOld.R")


        hopt<- -(HoptFun(FreqMatrixFinal, S) ) 
        return(hopt)

}

######### SIMULATED ANNEALING- TO FIND THE SEQUENCE THAT MINIMIIZES ENTROPY  ############      (9)

#### We want to find the minimum solution to the Entropy of the possible 10! = 3,628,800 sequence (of length 10) domain ####



######################### Simulated Annealing for Hopt ############################

SimAnnealHopt<-function(FreqMatrixFinal, Sint){
	Constant<- 1.011
	Scurrent<-Sint
	Sbest<-Scurrent
	Flag<-0; i<-1
	while(i<=150){		
      		i<-i+0.5
      		#print(i)
      		Si<-CreateneighbourSolNew(Scurrent)
      		tempcurrent<-CalculateTemp(Constant, i)
      		EntropySeqSi<-EntropySeqHopt(FreqMatrixFinal, Si); EntropySeqScurrent<-EntropySeqHopt(FreqMatrixFinal, Scurrent)
      		deltaEntropy<- EntropySeqSi-EntropySeqScurrent
      		if(deltaEntropy < 0){
			Scurrent<-Si
      			if(EntropySeqSi<=EntropySeqHopt(FreqMatrixFinal, Sbest)){
	    			#Flag<- Flag+1; #print(c("Flag=", Flag ,i))
	    			Sbest<-Si; #print(c("Flag=", Flag ,i, Sbest))
			}
			print(c("i=", i,-EntropySeqSi ))
			print(c("Scurrent", Scurrent))
			print(c("Sbest", Sbest))
      		}
      		else{
			if( exp(-deltaEntropy/tempcurrent)> runif(1,0,1) ) {
	    	    	    Scurrent<-Si; print(c("in else",exp(-deltaEntropy/tempcurrent), "temperature", tempcurrent))
			}
     		}

       }
      # return(Sbest)
       h<- -EntropySeqHopt(FreqMatrixFinal, Sbest)
       return(c(h, Sbest) )
}

\end{verbatim}
\end{comment}
}
